Parametric, Probabilistic, Timed Resource Discovery System

This paper presents a fully distributed resource discovery and reservation system. Verification of such a system is important to ensure the execution of distributed applications on a set of resources in appropriate conditions. A semi-formal model for his system is presented using probabilistic timed automata. This model is timed, parametric and probabilistic, making it a challenge to the parameter synthesis community.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{T. Brihaye, B. Delahaye, L. Jezequel, N. Markey, J. Srba (Eds.):\\
Cassting Workshop on Games for the Synthesis of Complex Systems\\
and 3rd International Workshop on Synthesis of Complex Parameters\\ 
(Cassting'16/SynCoP'16).\\
EPTCS 220, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.220.5}{10.4204/EPTCS.220.5}}
\pdfoutput=1

